Multimodal Metric Learning for Tag-based Music Retrieval

Tag-based music retrieval is crucial to browse large-scale music libraries efficiently. Hence, automatic music tagging has been actively explored, mostly as a classification task, which has an inherent limitation: a fixed vocabulary. On the other hand, metric learning enables flexible vocabularies by using pretrained word embeddings as side information. Also, metric learning has already proven its suitability for cross-modal retrieval tasks in other domains (e.g., text-to-image) by jointly learning a multimodal embedding space. In this paper, we investigate three ideas to successfully introduce multimodal metric learning for tag-based music retrieval: elaborate triplet sampling, acoustic and cultural music information, and domain-specific word embeddings. Our experimental results show that the proposed ideas enhance the retrieval system quantitatively, and qualitatively. Furthermore, we release the MSD500, a subset of the Million Song Dataset (MSD) containing 500 cleaned tags, 7 manually annotated tag categories, and user taste profiles.

==> Sec0_Supplimentary.tex <==
\section{Per tag AUROC on MTAT}

In Table~\ref{table:pertagauroc}, we report per tag AUROC on MTAT in a descending order. Note that our model is vulnerable to negative tags: `no voice', `no vocal', and `no vocals'.



\begin{table}[h!]
\centering
% \fontsize{7pt}{9pt}\selectfont
\small
\begin{tabular}{@{}ccccc@{}}
\toprule
metal        & choral & choir  & rock       & opera   \\
98.79        & 98.68  & 98.65  & 98.52      & 98.34   \\\midrule
flute      & harpsichord & cello        & techno    & dance    \\
97.91      & 97.85       & 96.61        & 96.51     & 96.08    \\\midrule
ambient      & piano  & harp   & country    & pop \\
95.69        & 95.69  & 95.12  & 94.05      & 94.01  \\\midrule
sitar      & man         & woman        & female    & beat     \\
93.99      & 93.70       & 93.53        & 93.41     & 93.23    \\\midrule
female vocal & male   & violin & male vocal & beats \\
92.99        & 92.91  & 92.62  & 92.34      & 92.25  \\\midrule
classical  & loud        & female voice & guitar    & quiet    \\
92.15      & 91.30       & 91.05        & 90.98     & 90.89    \\\midrule
solo         & drums  & indian & male voice & singing \\
90.36        & 89.99  & 89.99  & 89.79      & 89.77  \\\midrule
electronic & fast        & vocal        & new age   & classic  \\
89.37      & 89.15       & 88.81        & 88.73     & 88.66    \\\midrule
strings      & vocals & synth  & voice      & slow   \\
88.59        & 88.11  & 86.17  & 84.60      & 84.09   \\\midrule
soft       & weird       & no vocal     & no vocals & no voice \\
83.63      & 81.68       & 71.86        & 70.22     & 67.88    \\ \bottomrule
\end{tabular}
\vspace{0.3cm}
\caption{Per tag AUROC on MTAT}
\vspace{-0.5cm}
\label{table:pertagauroc}
\end{table}


% \begin{table*}[]
% \centering
% \fontsize{7pt}{9pt}\selectfont
% \begin{tabular}{@{}cccccccccc@{}}
% \toprule
% metal        & choral & choir  & rock       & opera   & flute      & harpsichord & cello        & techno    & dance    \\
% 98.79        & 98.68  & 98.65  & 98.52      & 98.34   & 97.91      & 97.85       & 96.61        & 96.51     & 96.08    \\\midrule
% ambient      & piano  & harp   & country    & pop     & sitar      & man         & woman        & female    & beat     \\
% 95.69        & 95.69  & 95.12  & 94.05      & 94.01   & 93.99      & 93.70       & 93.53        & 93.41     & 93.23    \\\midrule
% female vocal & male   & violin & male vocal & beats   & classical  & loud        & female voice & guitar    & quiet    \\
% 92.99        & 92.91  & 92.62  & 92.34      & 92.25   & 92.15      & 91.30       & 91.05        & 90.98     & 90.89    \\\midrule
% solo         & drums  & indian & male voice & singing & electronic & fast        & vocal        & new age   & classic  \\
% 90.36        & 89.99  & 89.99  & 89.79      & 89.77   & 89.37      & 89.15       & 88.81        & 88.73     & 88.66    \\\midrule
% strings      & vocals & synth  & voice      & slow    & soft       & weird       & no vocal     & no vocals & no voice \\
% 88.59        & 88.11  & 86.17  & 84.60      & 84.09   & 83.63      & 81.68       & 71.86        & 70.22     & 67.88    \\ \bottomrule
% \end{tabular}
% \vspace{0.3cm}
% \caption{Per tag AUROC on MTAT}
% \vspace{-0.5cm}
% \label{table:pertagauroc}
% \end{table*}


\section{More Results on Attention Heat Maps}

We report more attention heat maps of various types including voice (Figure~\ref{fig:attention_heatmap_voice}), mood (Figure~\ref{fig:attention_heatmap_mood}),  instrument (Figure~\ref{fig:attention_heatmap_inst}), and genre (Figure~\ref{fig:attention_heatmap_gnr}).

\section{Tag-wise Contribution Heat Maps}

More tag-wise contribution heat maps are illustrated in Figure~\ref{fig:tagwise_contrib_sub}.

\newpage
\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/male_1.png}
        \caption{Tag - Male}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/female_2.png}
        \caption{Tag - Female}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/vocal_1.png}
        \caption{Tag - Vocal}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/novocal_1.png}
        \caption{Tag - No Vocal}
    \end{subfigure}
    % \vspace{-0.2cm}
    \caption{Attention heat maps for voice tags.}
    \label{fig:attention_heatmap_voice}
    \vspace{-0.5cm}
\end{figure*}
\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/quiet_2.png}
        \caption{Tag - Quiet}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/loud_2.png}
        \caption{Tag - Loud}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/slow_1.png}
        \caption{Tag - Slow}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/fast_1.png}
        \caption{Tag - Fast}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/soft_1.png}
        \caption{Tag - Soft}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/weird_1.png}
        \caption{Tag - Weird}
    \end{subfigure}
    \caption{Attention heat maps for mood tags.}
    \label{fig:attention_heatmap_mood}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/cello_1.png}
        \caption{Tag - Cello}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/sitar_1.png}
        \caption{Tag - Sitar}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/harp_1.png}
        \caption{Tag - Harp}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/piano_2.png}
        \caption{Tag - Piano}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/strings_1.png}
        \caption{Tag - Strings}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/flute_1.png}
        \caption{Tag - Flute}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/drums_2.png}
        \caption{Tag - Drums}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/violin_1.png}
        \caption{Tag - Violin}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/guitar_1.png}
        \caption{Tag - Guitar}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/synth_1.png}
        \caption{Tag - Synth}
    \end{subfigure}
    \caption{Attention heat maps for instrument tags.}
    \label{fig:attention_heatmap_inst}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/classic_1.png}
        \caption{Tag - Classic}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/country_1.png}
        \caption{Tag - Country}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/opera_1.png}
        \caption{Tag - Opera}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/newage_1.png}
        \caption{Tag - New Age}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/rock_1.png}
        \caption{Tag - Rock}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/metal_1.png}
        \caption{Tag - Metal}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/pop_1.png}
        \caption{Tag - Pop}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/dance_1.png}
        \caption{Tag - Dance}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/electronic_1.png}
        \caption{Tag - Electronic}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/techno_1.png}
        \caption{Tag - Techno}
    \end{subfigure}
    \caption{Attention heat maps for genre tags.}
    \label{fig:attention_heatmap_gnr}
\end{figure*}




\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[h]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/female_male.png}
        \caption{Female + Male}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/classic_metal.png}
        \caption{Classic + Metal}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/vocal_no_vocals.png}
        \caption{Vocal + No Vocals}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/novoice_choir.png}
        \caption{No Voice + Choir}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/slow_fast.png}
        \caption{Slow + Fast}
    \end{subfigure}
    \begin{subfigure}[h]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/drums_harp.png}
        \caption{Drums + Harp}
    \end{subfigure}
    \caption{Tag-wise contribution heat maps.}
    \label{fig:tagwise_contrib_sub}
\end{figure*}

==> Sec5_Results.tex <==
% \section{Results}\label{sec:results}
% \subsection{Song Embeddings}
% Table~\ref{tab:songemb} reports the results of the experiment introduced in Section~\ref{subsec:song}. In general, a song embedding trained with acoustic information outperforms the embeddings trained with cultural information. However, in terms of P@10, cultural embeddings show competitive performance while other metrics are low. We observe that the predicted similarity of cultural embeddings has higher mean and variance than the similarity measured by acoustic embeddings. Cultural embeddings can make accurate decisions for the top few items but the prediction cannot generalize to low confidence items. We argue that this is because cultural information derived from the user taste profile has a relatively discrete boundary for a given tag while acoustic embeddings define a more linear similarity space. With a larger taste profile dataset, one can expect more linearity in the cultural embedding space since it may contain more diverse users and their listening history. On the other hand, the hybrid embedding, as we expected, performs best for every metric.

% Metrics reported in Table~\ref{tab:songemb} are averaged values over tag. To better understand the model, tag-wise analysis is important. 
% % \st{However, it is not intuitive to take a look at each individual tag because there are already 100 tags.} 
% To this end, we group tags into four different categories: genre, instrument, language/location, and mood. Note that we merge language and location together since they are not frequent in the top 100 tags. Figure~\ref{fig:tagwise} shows category-wise performance. Acoustic embeddings outperform the cultural ones except for language/location. This is because acoustic embeddings have to guess language/location tags since the source of the tags is not necessarily contained in the acoustic information. 

% Hybrid embeddings show lower performance than acoustic embeddings only for instrument tags. When we take a closer look at tag-wise metrics, the performance drop is only caused by the tag \textit{piano}. We suspect that cultural embeddings in our experiment, which use a relatively small user-item matrix compared to industry-level data, fail to generalize to the tag \textit{piano} because the nature of the tag is fully based on acoustic characteristics. Given the superiority of the hybrid embeddings, in the following sections we focus on their performance exclusively.
% % \textcolor{magenta}{
% %  Cultural low MAP, ROC-AUC. But high P@10.
% % Acoustic showed better result than Cultural.
% % Figure 2. But it depends on the tag type. Cutural worked better for language/location while Acoustic worked better for genre, instrument.
% % Of course, hybrid worked the best in Table 2.
% % But it's not always the best in Figure 2. Maybe because of the data skewness. 80 percents are genre tags.
% % }


% \begin{table}[t!]
% \centering
% \footnotesize
% \begin{tabular}{@{\hskip 0.12in}l@{\hskip 0.32in}c@{\hskip 0.32in}c@{\hskip 0.32in}c@{\hskip 0.12in}}
% \toprule
% Metrics & Cultural & Acoustic & Hybrid\\ \midrule
% MAP& 0.0656 & 0.0908 & \textbf{0.1050}\\
% P@10 &  0.1400  & 0.1430 & \textbf{0.1610}\\ 
% ROC-AUC& 0.7114 & 0.8263 & \textbf{0.8484}\\
%  \bottomrule
% \end{tabular}
% \caption{Performance of different embeddings on the proposed dataset.}
% \label{tab:songemb}
% \end{table}


% \begin{figure}
%  \centerline{
%  \includegraphics[width=0.97\columnwidth, trim=4 0 0 0, clip]{figs/inf.png}}
%  \caption{Category-wise MAP.}
%  \label{fig:tagwise}
% \end{figure}


% \subsection{Tag Embeddings}
% % \st{From here we only report the performance of hybrid embedding since we already know it works better than cultural or acoustic-only embedding. }
% As shown in Table~\ref{tab:word}, domain-specific word embeddings appear to perform better than the GloVe embeddings. ROC-AUC of domain-specific word embeddings is slightly lower but only marginally. Hence, injecting musical context in tag embeddings is beneficial for music retrieval. However, the versatility of this approach cannot be highlighted only with the proposed quantitative metrics. 
% % \st{We tried to check if the proposed domain-specific word embedding includes more musical context. We query}
% To this end, we check if these proposed domain-specific word embeddings include more musical information by querying with broader  music-related terms to retrieve top 10 nearest words. Examples of the top 10 nearest words can be seen in Table~\ref{tab:neighbor}. We embolden the retrieved tags that are music-related. As shown in the table, our domain-specific word embeddings handle queried words in a more musical context. This may facilitate richer vocabulary for users when they are allowed to query with free-form text.
% % \textcolor{magenta}{
% % Table 3. Music word embedding helps a bit. Only hybrid model.
% % It's power is not only the performance but also the vocabulary.
% % As shown in Table 4, it can cover more music related terms.
% % }





% \begin{table}[t!]
% \centering
% \footnotesize
% \begin{tabular}{@{\hskip 0.12in}l@{\hskip 0.12in}c@{\hskip 0.12in}c@{\hskip 0.12in}}
% \toprule
% Metrics & GloVe embedding & Domain-specific embedding\\ \midrule
% MAP& 0.1050 & \textbf{0.1118}\\
% P@10 &  0.1610  & \textbf{0.1800}\\ 
% ROC-AUC& 0.8484 & 0.8479\\
%  \bottomrule
% \end{tabular}
% \caption{Comparison of two different word embeddings.}
% \label{tab:word}
% \end{table}



% \begin{table}
% \centering
% \footnotesize
%  \begin{center}
% %  \begin{tabular}{|@{\hskip 0.08in}c|@{\hskip 0.08in}c|@{\hskip 0.08in}c|}
%  \begin{tabular}{|p{0.8cm}|p{2.8cm}|p{3.2cm}|}
%   \hline
%   Tag & GloVe embedding& Domain-specific embedding \\ \hline
%   House    & room, home, apartment, \textbf{party}, dad, office, coming, bedroom, next, out                   & \textbf{club}, \textbf{party}, \textbf{lounge}, kitchen, \textbf{jungle}, \textbf{dance}, \textbf{rave}, \textbf{parties}, \textbf{nightclub}, \textbf{club\_nights}                                      \\\hline
% Country    & america, american, states, town, southern, south, especially, way, africa, shame                   & traditional\_country, \textbf{bluegrass}, americana, \textbf{gospel}, \textbf{folk}, \textbf{cajun}, \textbf{honky\_tonk}, nashville, \textbf{rockabilly}, \textbf{honky-tonk}                                     \\\hline
% Chill    & chil, dude, forreal, yea, cool, relax, bruh, gotta, foreal, imma & \textbf{chill\_out}, relax, chilled, kick\_back, \textbf{chill-out}, relaxing, \textbf{chilled\_out}, \textbf{downtempo}, unwind, mellow                                       \\\hline
% % Brazilian    & portuguese, brazillian, peruvian, brazil, brazilians, italian, malaysian, argentine, argentinian, brasilian  & cuban, colombian, latin\_american, mpb, mariachi, latin, portuguese, mexican, bossa\_nova, brazilian\_popular                                      \\\hline
 
%  \end{tabular}
% \end{center}
%  \caption{10 nearest words of given tags in GloVe embedding and domain-specific word embedding.}
%  \label{tab:neighbor}
% \end{table}



% \subsection{Data Sampling}
% From here on we only report the results using hybrid embeddings in the song embedding branch and domain-specific word embeddings in the tag embedding branch. We compare a simple random triplet sampling method with our proposed triplet sampling introduced in subsection~\ref{subsec:sampling}. As reported in Table~\ref{tab:sample}, our balanced triplet sampling approach shows a dramatic performance gain. The impact of data sampling is the biggest among the three different challenges discussed in this paper.
% To demonstrate the importance of elaborated data sampling, we visualize the MAP curve on the validation set in Figure~\ref{fig:curve}. The orange curve is random sampling and the blue curve is our balanced sampling. Since our balanced sampling method guarantees equal chances for minor tags to be sampled during training, it successfully reduces the search space. Thanks to this, the model can skip redundant and less informative triplets, and thus, representation learning is accelerated.
% % If we compare with the performance of the baseline model~\cite{choi2019zero} (i.e., Table~\ref{tab:songemb} Acoustic), our proposed considerations doubled the MAP of cross-modal retrieval model.



% \begin{table}[t!]
% \centering
% \footnotesize
% \begin{tabular}{@{\hskip 0.12in}l@{\hskip 0.12in}c@{\hskip 0.12in}c@{\hskip 0.12in}}
% \toprule
% Metrics & Random sampling & Balanced sampling\\ \midrule
% MAP& 0.1118 & \textbf{0.1821}\\
% P@10 &  0.1800  & \textbf{0.3520}\\ 
% ROC-AUC& 0.8479 & \textbf{0.8853}\\
%  \bottomrule
% \end{tabular}
% \caption{Performance of different sampling methods.}
% \label{tab:sample}
% \end{table}


% \begin{figure}
%  \centerline{
%  \includegraphics[width=0.97\columnwidth, trim=4 0 0 0, clip]{figs/curve.png}}
%  \caption{Validation MAP curves of different sampling methods during training.}
%  \label{fig:curve}
% \end{figure}

% \begin{figure}
%  \centerline{
%  \includegraphics[width=0.97\columnwidth, trim=4 0 0 0, clip]{figs/ft.png}}
%  \caption{Figure captions should be placed below the figure.}
%  \label{fig:tagwise}
% \end{figure}


